Deciphering Refactoring Branch Dynamics in Modern Code Review: An Empirical Study on Qt

Context: Modern code review is a widely employed technique in both industrial and open-source projects, serving to enhance software quality, share knowledge, and ensure compliance with coding standards and guidelines. While code review is extensively studied for its general challenges, best practices, outcomes, and socio-technical aspects, little attention has been paid to how refactoring is reviewed and what developers prioritize when reviewing refactored code in the Refactor branch. Objective: The goal is to understand the review process for refactoring changes in the Refactor branch and to identify what developers care about when reviewing code in this branch. Method: In this study, we present a quantitative and qualitative examination to understand the main criteria developers use to decide whether to accept or reject refactored code submissions and identify the challenges inherent in this process. Results: Analyzing 2,154 refactoring and non-refactoring reviews across Qt open-source projects, we find that reviews involving refactoring from the Refactor branch take significantly less time to resolve in terms of code review efforts. Additionally, documentation of developer intent is notably sparse within the Refactor branch compared to other branches. Furthermore, through thematic analysis of a substantial sample of refactoring code review discussions, we construct a comprehensive taxonomy consisting of 12 refactoring review criteria.

==> Sections/08_DataAvailability.tex <==
%\section{Data Availability}
%\label{Section:dataavailability}


==> Tables/RQ1_statistics.tex <==
\begin{table}
  \centering
\caption{Results of Mann-Whitney U test and effect size for refactoring and non-refactoring code reviews.}
\label{Table:RQ1_statistical_test}
%\begin{sideways}
%\begin{sideways}
\begin{adjustbox}{width=0.5\textwidth,center}
%\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{llll}\hline
\toprule
\bfseries Metric &  \bfseries \textit{p}-value & \bfseries Cliff's delta ($\delta$)  \\
\midrule
Number of reviewers  &   \textbf{6.750458e-43} & small (0.15)
\\ 
Number of review comments  & \textbf{2.730193e-82} & small (0.22)
\\
Number of inline comments &  \textbf{2.066649e-98} & medium (0.33)
\\
Number of revisions &   \textbf{1.252695e-126} & small (0.3) 
  
\\
Number of changed files &   \textbf{6.006899e-190} & medium (0.33)

\\
Review duration  &   \textbf{2.572584e-66} & small (0.23)

\\
Length of discussion &   \textbf{6.966752e-42} & small (0.15)

\\
Length of description &   \textbf{4.071541e-41} & small (0.13)
  
\\ 
Code churn &   \textbf{0.000000e+00} &  large (0.64)

\\
\bottomrule
\end{tabular}
\end{adjustbox}
%\end{sideways}
\end{table}

==> Tables/RelatedWork_CodeReview.tex <==
\begin{table*}
  \centering
  %\fontsize{8}{9}\selectfont
	%\tabcolsep=0.05cm
	 \caption{Related work in refactoring-related code review.}
	 \label{Table:Related_Work_in_Refatoring_Code_Review}
%\begin{sideways}
\begin{adjustbox}{width=1.0\textwidth,center}
\rowcolors{2}{white}{gray!25}
%\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{lclllll}\hline
\toprule
\bfseries Study & \bfseries Year  &  \bfseries Research Type & \bfseries Research Method & \bfseries Purpose & \bfseries Evaluation Technique  \\
\midrule
Ge \etal  \cite{ge2014towards,ge2017refactoring} & 2014,2017 & Tool-based code review & Case \& formative study & Detect refactoring from non-refactoring changes & 2 OSS \& 35 developers  \\ 
Alves \etal  \cite{alves2014refdistiller,alves2017refactoring} & 2014,2018 & Tool-based code review & User study & Inspect manual refactoring edits & 3 OSS \& 15 developers \\ 
Morales \etal  \cite{morales2015code} & 2015 & Empirical study & Case study  & Understand the impact of code review on quality &  3 OSS \\ 
Coelho \etal  \cite{coelho2019refactoring} & 2019 & Literature review & Systematic mapping study & Present refactoring solutions to MCR & N/A \\
Pascarella \etal  \cite{DBLP:journals/corr/abs-1912-10098} & 2019 & Empirical study & Case study & Study the effect of code review on code smells &  7 OSS  \\ 
Paix{\~a}o \etal  \cite{paixao2020behind} & 2020 & Empirical study & Mining-based & Study refactoring in MCR  & 6 OSS\\ 
Pantiuchina \etal \cite{pantiuchina2020developers} & 2020 &  Empirical study & Mining-based & Study refactoring in pull requests  & 150 OSS \\
Uch{\^o}a \etal \cite{uchoa2020does} & 2020 & Empirical study & Mining-based & Study MCR \& design degradation & 7 OSS\\ 
Uch{\^o}a \etal \cite{uchoa2021predicting} & 2021 & Empirical study & Mining-based & Predict design impactful changes in MCR & 7 OSS \\ 
AlOmar \etal \cite{alomar2021icse} & 2021 & Empirical \& industrial case study  & Case study \& survey & Understand refactoring challenges in MCR & 24 developers \\
Brito \& Valente \cite{brito2020refactoring} & 2021 &  Tool-based code review & User study & Detect refactoring during code review & 8 developers\\
Kurbatova \etal \cite{kurbatova2021refactorinsight} & 2021 & Tool-based code review & Mining-based &  Enhance IDE representation
of changes & 4 OSS \\
Coelho \etal \cite{coelho2021empirical} & 2021 &  Empirical study & Mining-based & Study refactoring-inducing pull requests  &  350 OSS \\
AlOmar \etal \cite{alomar2022code} & 2022 & Empirical \& case study & Mining-based & Understand refactoring practices in MCR & 2,225 OSS \\


\bottomrule
\end{tabular}
\end{adjustbox}
%\end{sideways}
\vspace{-.3cm}
\end{table*}
